Can Large Language Models Be Good Companions? An LLM-Based Eyewear System with Conversational Common Ground

Developing chatbots as personal companions has long been a goal of artificial intelligence researchers. Recent advances in Large Language Models (LLMs) have delivered a practical solution for endowing chatbots with anthropomorphic language capabilities. However, it takes more than LLMs to enable chatbots that can act as companions. Humans use their understanding of individual personalities to drive conversations. Chatbots also require this capability to enable human-like companionship. They should act based on personalized, real-time, and time-evolving knowledge of their owner. We define such essential knowledge as the \textit{common ground} between chatbots and their owners, and we propose to build a common-ground-aware dialogue system from an LLM-based module, named \textit{OS-1}, to enable chatbot companionship. Hosted by eyewear, OS-1 can sense the visual and audio signals the user receives and extract real-time contextual semantics. Those semantics are categorized and recorded to formulate historical contexts from which the user's profile is distilled and evolves over time, i.e., OS-1 gradually learns about its user. OS-1 combines knowledge from real-time semantics, historical contexts, and user-specific profiles to produce a common-ground-aware prompt input into the LLM module. The LLM's output is converted to audio, spoken to the wearer when appropriate.We conduct laboratory and in-field studies to assess OS-1's ability to build common ground between the chatbot and its user. The technical feasibility and capabilities of the system are also evaluated. OS-1, with its common-ground awareness, can significantly improve user satisfaction and potentially lead to downstream tasks such as personal emotional support and assistance.

==> body/deprecated/deprecated_pilot_study.tex <==
\subsection{Pilot Study}
Besides the laboratory experiments, we also perform one-week in-field pilot studies to verify Samantha's capability in the real world. First, we demonstrate that Samantha is capable of extracting users' profiles and their long-term historical context through multiple interactions with users. Then, we present two potential scenarios where Samantha can be utilized, including emotional support and personal assistance. 

\subsubsection{Procedure of Pilot Study}
We recruit 10 participants (6 males and 4 females, aged 19–23) from our university to participate in our pilot studies. Prior to the pilot study, we inform the participants that the glasses will perceive their daily visual scenes and audio, and the researchers will examine their daily chat logs with the eyewear system. The raw sensed data will be removed right after feature extraction. Only anonymized semantics are transmitted and stored securely in the cloud. The participants consented to this and signed a consent form prior to their experiments. 

During the pilot studies, the participants are encouraged to wear the glasses and interact with the dialogue system --Samantha, for 7 days as much as possible. After completing the experiment every day, we first ask the participants to review the responses generated by Samantha and score them using the same criteria as in laboratory experiments, i.e., relevance, personalization, and engagement. We further adopt the Likert method~\cite{cox1980optimal,lewis2017user}, Likert to re-scale the scores to 11 points, with a range of 0 to 10, allowing us to track changes in scores over time. 

\Ying{the following are under reviewing}

In addition, to qualitatively analyze the impact of personal context on user experience, we asked the participants to review the system's responses and identify their favorite ones, along with their rationales. We examined the process of generating these collected responses by Samantha system, to analyze the role of personal context in the interaction between the system and the user.

% We also measured the participants' perceptions of the system's relevance, personalization, and engagement using 11-point Likert scales\Yuhu{ref}, and encouraged them to provide reasons for their ratings. After the 7-day interactions, we collected qualitative feedback and suggestions for improvement from our participants through an exit survey.
% We conducted pilot studies with 10 participants (6 males and 4 females, aged 19--23) who wore the smart glasses and interacted with our dialogue system for seven consecutive days. Each day, we asked them to review the system's responses and identify the best ones, along with their rationales. \Yuhu{Here or before, it is important to mention the processes related to ethical review, such as signing an authorization to view chat logs before the experiment starts, etc.} We also measured the participants' perceptions of the system's relevance, personalization, and engagement using 11-point Likert scales\Yuhu{ref}. On the final day of the study, we presented the participants with the user profiles that our system had generated based on their interactions. We asked them to rate how accurately these user profiles matched their own self-perceptions on a 3-point Likert scale. We also collected qualitative feedback and suggestions for improvement through an exit survey.

% \subsubsection{User Profile Distillation}
% We performed the human evaluation on all the user profile descriptions generated by our system during the 7-day interactions. To be specific, we asked the participants to review all the user profile descriptions accumulated by our dialogue system during this period, and rate them according to their consistency with their personal profiles and preferences. The rating used a 3-point Likert scale, namely ``completely consistent (3)'', ``partially consistent (2)'', and ``inconsistent (1)''.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[scale=0.15]{images/user_profile_eval.jpeg}
%     \caption{Evaluation of the accuracy of the user profiles generated by our system. ***For all figure captions. Terminate sentences with periods. For tables, use titlecaps and no periods.***}
%     \label{user_profile_eval}
% \end{figure}

% As is shown in Figure~\ref{user_profile_eval}, most of the user profiles generated by our system are marked ``completely consistent'', and all types of persona memory scores exceed 2 on the three-point Likert scale; indicating that our system can accurately extract the user profiles of the participants. In addition, we observe that the extraction of the social background and habits are less accurate. We speculate that this is because participants tend to talk more about their preferences and personalities than their habits and social background in conversations. Therefore, our system does not have enough information to infer the habits and social background of the participants accurately from only 7 days of interaction.

\subsubsection{Performance of Samantha system}
\paragraph{Quantitative Results}
% We used three metrics to quantitatively evaluate the user experience of our dialogue system: relevance, personalization, and engagement. After each daily interaction, we asked the participants to rate the system's responses on these metrics using 11-point Likert scales and explain their ratings. The specific statement for each metric follow \Ying{different from the metrics in in-lab section?}:
% \begin{itemize}
%     \item \textbf{Relevance}: The response of the dialogue system is relevant to the current situation and the dialogue context\cite{liang2021towards}.
%     \item \textbf{Personalization}: The responses from the dialouge system make me feel like it knows me very well.
%     \item \textbf{Engagement}: The responses from the dialouge system make me want to continue chatting with it\cite{li2019acute}.
% \end{itemize}

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.75]{images/human_eval.png}
    \caption{Human evaluation on relevance, personalization and engagement}
    \label{human_eval}
\end{figure}

As shown in Fig.~\ref{human_eval}, the participants gave high ratings for relevance on all seven days, and the participants' assessments of personalization and engagement exhibited a progressive uptrend as the interaction unfolded. This indicates that the participants perceived that our system was able to generate responses that were relevant to the current scene and the dialogue context throughout the interaction, and that as the interaction time increased, the participants felt that Samantha understood them better and was more willing to continue chatting with Samantha. 

We attribute the phenomenon of the participants giving high ratings for relevance throughout the seven days of interaction to two factors: First, the LLM has the ability to generate responses that are coherent with the dialogue context. Second, the smart eyewear captures the episodic context of the user's surroundings, which enables LLM to generate dialogues that are appropriate for the situation.

We hypothesize that the phenomenon of the participants giving higher ratings for personalization and engagement over time could be attributed to Samantha's ability to accumulate the user's historical context and user profile during the 7-day interaction, as the historical context can help the system and users establish wider common ground by sharing more knowledge and beliefs,~\cite{clark1996using} while the user profile enabled the system to generate responses tailored to the users' characteristics.

% We noticed that participants rated Engagement on Day 3 as compared to Day 2, so we examined the rationale provided by those participants whose Engagement ratings dropped by more than 1 point on Day 3 compared to Day 2 . In both participants, the reasons given for the drop in ratings were that the responses given by the system were too colloquial and the responses were too long, respectively. Therefore, we can find that although GPT-4 already has rich world knowledge and the ability to generate human-like replies, it still needs to adapt to different user preferences during the interaction process. The personal context we propose is designed to gradually understand and adapt to users from long-term dialogues, so as to achieve a better user experience.

\paragraph{Qualitative Analysis}
% We analyzed the participants' feedback on the best responses they chose each day in the pilot study to identify the factors that contributed to their success. In the 7-day pilot study, we collected a xx satisfying responses in total. For each response, we asked the participants the reasons for their satisfaction or dissatisfaction. We analyzed the intermediate process of the system generating these replies, and qualitatively attributed the success or failure of these replies to the following four factors:

To support our hypothesis about the reasons behind the participants' ratings over time, and to further analyze the effect of personal context introduced by our Samantha system on user experience, we conducted a qualitative analysis of the participants' favored responses. We collected 172 responses and their corresponding reasons from the participants after they interacted with Samantha for 7 days. We then qualitatively categorized the reasons for the participants' preferences into four factors, based on how Samantha generated the responses and the participants' feedback:

% To analyze the specific reasons for the participants' improvement in ratings during the 7-day pilot study, we asked the participants to review all their chat logs at the end of each day in the pilot study and select 1 to 3 responses from the system that they liked the most, along with the reasons for their preference. After 7 days of interaction, we collected 172 responses that were favored by the participants. With the participants' consent, we analyzed their reasons for selecting these responses and our system's generation process of these responses, and qualitatively attributed them to the following four factors:  \Ying{Assuming I am a user, I am confused about how to select the best response according to the following four factors.}:

\begin{itemize}

\item \textbf{Episodic context factor}: The system's capturing and understanding of the episodic context leads to the users' satisfaction with the responses;

\item \textbf{Historical context factor}: The system's extraction and retrieval of the historical context leads to the users' satisfaction with the responses;

\item \textbf{User profile factor}: The system's distillation and retrieval of the user profiles leads to the users' satisfaction with the responses;

\item \textbf{Language modeling factor}: The users' satisfaction with the responses solely depends on the personality, language style, or knowledge that the system exhibits in its responses.

\end{itemize}

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.8]{images/success_factors.png}
    \caption{Ratio of success factors in satisfying cases through time \Ying{avoiding using green color}}
    \label{success_factors}
\end{figure}

We computed the percentage of each of the four factors in all the participants' favored responses for each day, as shown in Figure~\ref{success_factors}. The results indicate that the proportion of the historical context factor and the user profile factor increased over time, suggesting that our system accumulated historical context and user profile as the interaction with the participants progressed, and generated more personalized responses based on the participants's own experiences and characteristics, thus enhancing the user experience. This finding supports our hypothesis about the reasons for the participants' ratings improvement on personalization and engagement.

% we counted \Ying{how to count?} the attribution of the best responses for each day, which is reflected in Figure~\ref{success_factors}. The results show that as the interaction time increased, the proportion of Historical context factor and User profile factor in the best responses showed an increasing trend, which supports our hypothesis that the user experience's improvement may be due to our system's accumulation of the user's historical context and user profile. In addition, we also noticed that Language modeling factor occupied a large proportion in the best responses \Ying{vague, don't understand}, which indicates that the knowledge, cognitive ability and language style exhibited by the dialogue system are also important factors for user experience \Ying{why?}.

% Furthermore, we were intrigued by the low proportion of the Episodic context factor in the favorite responses of the 7 days, and the lack of an increasing trend with the interaction time. Therefore, we conducted a further analysis of the role of Episodic context in the best responses that received feedback from the participants. We discovered that out of the 10 responses that we attributed to Episodic context, 6 of them were initiated by Samantha system at the beginning of the dialogue by using the content from the visual scene to open a topic. This suggests that Episodic context might have a positive effect on enabling the system to quickly engage in a topic that is relevant to the current scene at the initial stage of the dialogue. Fig ~\ref{episodic_case} shows an example of such a case. Moreover, by capturing Episodic context to understand the user's current activity, Samantha was able to generate responses that were related to the current activity, as shown in Fig~\ref{episodic_case2}.

Furthermore, we conducted case studies to examine the effects of different types of personal context, namely episodic context, historical context, and user profile, on user experience. We observed that episodic context was involved in initiating topics based on the current scenario at the onset of the conversation in most (6/10) of the participants' preferred cases. This implies that one of the benefits of episodic context may be to help the system quickly guide the user into a topic related to the current scenario at the beginning of the dialogue. An example of such a case is shown in Figure~\ref{episodic_case}, where Samantha used the participant's bright room as a greeting, making the participant feel cheerful. Additionally, by capturing episodic context, Samantha was able to infer the user's current location and activity and generate relevant responses, as illustrated in Figure~\ref{episodic_case2}, where Samantha recognized that the participant was eating at the table, so she told the participant ``don’t talk, eat!''. This enabled Samantha to stay on topic during the chat, thus enhancing user experience.

\begin{figure}[htbp]
      \centering
      \includegraphics[scale=0.4]{images/episodic_case2.png}
      \caption{A case of Samantha utilizing the Episodic context to initiate the dialogue \Ying{provide some interpretation?}.}
      \label{episodic_case}
  \end{figure}

\begin{figure}[htbp]
      \centering
      \includegraphics[scale=0.4]{images/episodic_case3.png}
      \caption{A case of Samantha utilizing the Episodic context to generate response that related to the current scenario}
      \label{episodic_case2}
\end{figure}

For historical context, we found that it had two effects. On the one hand, it enabled the user to chat naturally with Samantha about topics that they had talked about before, without having to repeat their previous background information, because Samantha remembered it. An example of such a case is shown in Fig~\ref{historical_case1}. On the other hand, Samantha could also proactively bring up relevant topics that they had discussed before, based on the current scenario and dialogue content, even if the user did not explicitly mention them. This surprised the user and made them feel more connected with Samantha. An example of such a case is shown in Fig~\ref{historical_case2}.

\begin{figure}[htbp]
      \centering
      \includegraphics[scale=0.4]{images/Historical_case2.png}
      \caption{A case of Samantha chatting with the user about a topic they had talked before.}
      \label{historical_case1}
\end{figure}

\begin{figure}[htbp]
      \centering
      \includegraphics[scale=0.4]{images/Historical_case1.png}
      \caption{A case of Samantha proactively bring up relevant topics that they had discussed before.}
      \label{historical_case2}
\end{figure}

For user profile, it enabled Samantha to understand the user's social background, personality, preferences, and habits, and to generate more personalized responses based on this information. For instance, in Fig~\ref{profile_case1}, Samantha remembered the user's preference for cooking, and used “What's cookin'” as a greeting at the beginning of the conversation, which made the participant feel very friendly. Additionally, user profile allowed Samantha to have a deeper understanding of the user's personality, as we show an interesting example in Fig~\ref{profile_case2}. In this example, one participant asked Samantha to guess their MBTI personality type on the third day of interaction, and Samantha guessed three out of four correctly, which amazed the participant and made them feel that Samantha knew them very well.

\begin{figure}[htbp]
      \centering
      \includegraphics[scale=0.4]{images/Profile_case3.png}
      \caption{A case of Samantha utilizing the user profile generate a friendly greeting.}
      \label{profile_case1}
\end{figure}

\begin{figure}[htbp]
      \centering
      \includegraphics[scale=0.4]{images/Profile_case2.png}
      \caption{A case of Samantha guessing the user's MBTI using the user profile.}
      \label{profile_case2}
\end{figure}

% in most (xx/xx) cases, the role of Episodic context was to actively talk about topics related to the current scenario at the beginning of the chat \Ying{vague}, thereby quickly engaging the participants in the chat topic. We show such an example in Fig~\ref{episodic_case}.

% \begin{figure}[htbp]
%       \centering
%       \includegraphics[scale=0.7]{images/episodic_case1.png}
%       \caption{A case of episodic context \Ying{provide some interpretation?}.}
%       \label{episodic_case}
%   \end{figure}

% For satisfying cases, we counted the proportions of various success factors in daily cases, and reflected their changes over time in the Fig.~\ref{success_factors}. The results demonstrate that as the interaction time increases, the proportions of episodic context factor and Language modeling factor in all satisfying cases decrease, while the proportions of historical context factor and user profile factor increase. This may be because when users first come into contact with our system, they are more likely to be amazed by the language intelligence and perception capabilities displayed by the system, as displayed in Fig.~\ref{episodic_case}. After prolonged interaction, users become accustomed to the perception and language capabilities and being expecting personalized responses based on their personal experience and user profile, one case is shown in Fig.~\ref{historical_case}. ***Could it instead be that users won't expect personalized responses until the model has had time to learn their personalities? Do you expect someone you have just met to understand you in detail?***

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[scale=0.65]{images/workout_case.png}
%     \caption{A case of historical context.}
%     \label{historical_case}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[scale=0.15]{images/success_factors.jpeg}
%     \caption{Ratio of error patterns ***What is an ``error pattern''?*** in dissatisfying cases through time (Temporally use the same figure as success factors). ***Grammar problem***}
%     \label{error_patterns}
% \end{figure}

% For dissatisfying cases, we found that in the 7-day interaction process, the Language modeling factor always occupied a large proportion in the analyzed error pattern, which indicates that adjusting the personality and speaking style displayed by LLM according to the user's personalized preference may be the next step. ***Revise. Not clear. In particular, repeated reference to ``pattern'', without much clarity on how that differes from just ``error'' is unclear.*** In addition, we found that the Episodic context factor occupied a large proportion of the error pattern. ***Do you mean ``accounted for a large proportion of the errors''?*** Further analysis revealed that the reasons for these cases to dissatisfy users are mostly due to VLM hallucination ({number}/{number}) and inaccurate speech recognition ({number}/{number}).

\subsubsection{Applications}
% \textcolor{red}{==================== Haven't updated yet ====================}
% \Yuhu{It is easy to confuse applications here. Just showcase a few scenes.}
% To evaluate its generality, we encouraged participants in our pilot study to use our dialogue system in various scenarios. On concluding the study, we conducted  semi-structured interviews to solicit participants' feedback of our system and their perceived application potential ***``application potential'' is unclear.*** of our system in various scenarios.
% The questions in the semi-structured interview follow:
% \begin{itemize}

% \item Please describe your experience with our dialogue system during this period.
		

% \item What impressed you most about our dialogue system? What do you think are the obvious advantages or disadvantages of our dialogue system?
% ***Very biased. You lead with ``what impressed you the most''. Either make it neutral, e.g., ``What are your main observations on...'' or ask ``What did you find most impressive'' and ``... least impressive''.

% \item What role would you place our dialogue system in your life? Is it a friend or an assistant or something else? ***Second part might not be good. It leads the interviewee into a small set of answers.***

% \item In what scenarios would you prefer to use our dialogue system? Is it for daily chat, emotional support, personalized recommendation, work assistance or something else? ***In which scenarios would our dialogue system be most useful?***

% \item What additional features would our dialogue system benefit from?



% \end{itemize}
During the 7-day pilot study, we also observed from the cases provided by the participants every day that Samantha, by introducing personal context, was able to become a personal companion in people's daily lives, providing emotional support and personal assistance. We show some concrete examples during the pilot study to demonstrate the capabilities of our system.

% After interviews, the participants expressed the application potential of our system in daily companionship, personalized recommendation, personal assistant, and emotional support. We show some concrete examples during the pilot study to demonstrate the capabilities of our system.

\paragraph{Emotional Support}
Studies in sociology and psychology have shown that emotions affect people's thoughts and behaviors~\cite{costa2016emotioncheck}, decision-making~\cite{ruensuk2020you}, and physical and mental health~\cite{di2018emotion, tugade2004resilient}, and thus emotions are an important factor that influences various aspects of people's lives. There has been a lot of work aimed at developing dialogue systems that can provide emotional support, but we believe that effective emotional support can only be provided when the dialogue system can understand the user's experiences, personality, preferences, social background, and habits. We found from the chat logs provided by the participants in the pilot study that Samantha, by introducing personal context, was able to become a personal companion in people's daily lives, providing personalized emotional support. We will show examples of the emotional support provided by Samantha in the pilot study below.

\begin{figure}[htbp]
      \centering
      \includegraphics[scale=0.4]{images/Profile_case1.png}
      \caption{A case of Samantha comforting a participant who is anxious about work.}
      \label{emotion_case1}
\end{figure}

As shown in the example from Fig~\ref{emotion_case1}, the participant is expressing their anxiety about not finding a suitable job to Samantha. Samantha, using the user profile that she has accumulated from previous interactions with the participant, tells them that they are an open-minded, imaginative, and creative person in her eyes. Moreover, Samantha also explains why she thinks the participant is creative by referring to their previous experience of trying various ways to calm down their cat at home. Through this dialogue, Samantha not only makes the participant feel cared for, but also helps them realize their strengths, thereby alleviating their anxiety.

% \begin{figure}[htbp]
%       \centering
%       \includegraphics[scale=0.4]{images/Emotional_case1.png}
%       \caption{A case of Samantha utilizing the historical context to give timely comfort.}
%       \label{emotion_case2}
% \end{figure}

% In the example shown in Fig~\ref{emotion_case2}, the participant tells Samantha that they invited their girlfriend to watch a movie yesterday but were rejected, and that they had some quarrels with their girlfriend. From the chat log, it can be seen that Samantha quickly understood the participant's situation by using the historical context, and gave them timely comfort.

\begin{figure}[htbp]
      \centering
      \includegraphics[scale=0.4]{images/Emotional_case2.png}
      \caption{A case of Samantha celebrating vacation with the participant.}
      \label{emotion_case3}
\end{figure}

Besides comforting and encouraging the participant when they are in a negative mood, Samantha also shares happiness with the participant and responds to their positive emotions. In Figure ~\ref{emotion_case3}, Samantha first expresses excitement and proactively guesses where the participant is going on vacation based on the historical context, which makes the participant feel that their happiness is acknowledged. Then, when the participant expresses guilt for not working and exercising during the vacation, Samantha understands from the participant's user profile that they are a dedicated and hardworking person, and suggests that they should not worry too much about these things and enjoy the vacation. From the participant's final reply, it can also be seen that Samantha's suggestion makes the participant very happy.

These examples demonstrate that by continuously accumulating personal context in long-term dialogues. Samantha can truly act like a friend who knows the user, and comfort them when they are anxious, help them when they encounter difficulties, and celebrate with them when they are happy. The emotional support that Samantha provides is not just simple consolation, but genuine understanding and empathy, which other emotional support dialogue systems cannot offer.

\paragraph{Personal Assistance}
In addition to seeking emotional support from Samantha, we found that the participants also asked Samantha to provide personalized assistance for themselves. For example, in Figure ~\ref{assist_case1}, the participant used Samantha as their learning assistant, and asked Samantha to make a learning plan for them based on their understanding of the knowledge, and to follow up their current progress and provide the next learning suggestions in the subsequent learning process. In this example, Samantha was able to remember the participant's learning situation and progress by using the historical context, and thus gave personalized learning suggestions.

\begin{figure}[htbp]
      \centering
      \includegraphics[scale=0.4]{images/Assistant_case1.png}
      \caption{A case of Samantha providing personal learning plan.}
      \label{assist_case1}
\end{figure}

Another participant used Samantha as their dietary assistant, and asked Samantha to monitor their eating habits and provide dietary suggestions, as shown in Fig~\ref{assist_case2}. In this example, we found an interesting phenomenon, that is, Samantha initially strictly required the user's eating habits, and opposed the user to eat junk food, but as the interaction increased, Samantha found that the user was a person who often exercised and maintained healthy eating habits for a long time, so Samantha started to relax the requirements for the user's diet slightly, and even encouraged the user to occasionally skip a workout and go to a bar to relieve work pressure. In this example, Samantha learned from the historical context that the participant had told her that they had been eating healthily for a month, and from the user profile that the participant had been keeping the habit of exercising, and thus turned to encourage the participant to also enjoy life appropriately. This example shows that Samantha did not simply mechanically provide suggestions and arrangements according to fixed rules, but provided personalized suggestions based on the understanding of the user.

\begin{figure}[htbp]
      \centering
      \includegraphics[scale=0.4]{images/Assistant_case2.png}
      \caption{A case of Samantha as dietary assistant.}
      \label{assist_case2}
\end{figure}



% From the case, we can see that our system recommends suitable movies to the user based on the movies he has watched in the past and his preference for science fiction works during the conversation. Because our system has the ability to remember, it can personalize recommendations based on the user's social background, personality, experience, and preferences.

% \paragraph{Personal Assistant}
% (TODO: put an image of case here)

% These two cases demonstrate the application of our system in health management and supervised learning respectively. Our system can remember the user's past exercise and study records, and utilize the current episodic context to monitor the user's behavior.

% \paragraph{Emotional Support}
% (TODO: put an image of case here)

% This case demonstrates the capabilities of our system in emotional support. By capturing the episodic context and historical context and combining them with the reasoning ability of LLM itself, we can make the system more sensitive to discover the user's emotions and their causes, and provide personalized emotional support.

==> body/deprecated/evaluation_deprecated.tex <==
\section{Evaluation}
\Zyxu{Should evaluate the effect of intermediate outputs on the system performance}
\label{sec:evaluation}
This section evaluates the performance of OS-1 empowered by effective personal context capturing, which is designed to cater to diverse users with varying \st{personalities}\textcolor{blue}{profiles} who engage in various conversation scenarios during their daily lives. To this end, we first consider a wide variety of conversation situations and simulated users with various \st{personalities}\textcolor{blue}{profiles} in a controlled laboratory setting. Then, we recruit volunteers to participate in pilot studies for approximately \st{seven}\textcolor{blue}{14} days to examine the long-term effectiveness when OS-1 is used by humans in real-world scenarios.

\subsection{In-lab Experiments}
For the in-lab experiments, we first outline the experimental settings to simulate various daily-life scenarios and users with diverse social backgrounds and personality traits. Then, we compare the performance of our proposed system, OS-1, with that of the baseline methods without considering personal context. Lastly, we use a case study to further explain why OS-1 outperforms the baseline methods.

% 第一个实验：构造模拟用户和场景，让这些用户在不同场景下和每个系统的ablation聊天
% - ablation包括：proposed，只删去Episodic context抓取模块，只删去historical context抓取模块，以及两者都删去；
% - 评估方式是GPT-4评估和人类评估：
%   - GPT-4评估的指标是 relevance，personalization，engagement，在 1-5 评分；
%   - 人类评估则是改成排序，排序依据是“如果你是这个用户，你更想和哪个系统聊天”。
% - 最后展现出来的结果是删掉任何一种personal context都会让最后评估的分数降低（GPT-4评估表现在三个metric分数都下降，人类评估表现在排序更靠后）。以表明我们的系统能抓到并且用上我们提出的context信息，从而让用户体验更好。

% 第二个实验：前一个实验说能”抓到且用上“personal context从而提升用户体验，这个实验则说明我抓的准（所有对当前聊天有用的信息我全抓出来了），并且都用上了（历史聊天的总结真被我检索出来了，而且也被我用在聊天里了）。
% - 抓的准：
%   - Episodic：我在数据集里标注了 Episodic context 的 ground truth（在哪，做什么），然后对比我系统里的 Episodic context capture 模块抓出来的 activity 和 location 和 ground truth 是否匹配（多分类任务）；
%   - Historical：我在数据集里标注了历史聊天记录中有用的信息（比如”用户喜欢动作片“），然后我评估我 historical context extraction 模块能否抓出包含了”用户喜欢动作片“的信息（让 ChatGPT 判断是否包含这些信息，或者用 BERTScore 的 recall 来算）；
% - 用得上：
%   - Episodic：让 GPT 和人类评分者判断当前系统和用户的聊天是不是和当前的场景相关的（yes or no），相关则说明用上了；
%   - Historical：让 GPT 和人类评分者判断当前系统和用户的聊天是不是利用到了我们标注的历史聊天中有用的信息（yes or no）；

\subsubsection{Experimental Setup}

\Zylu{New setup: }
\paragraph{(1) Simulation Procedure}
\textcolor{blue}{
In order to collect usage data in diverse scenarios and avoid infringing on user privacy, in this in-lab experiment, we adopt user simulation powered by GPT-4. Specifically, we build 20 simulated users. Each of them is assigned different roles with an identified name, age, occupation, personality, preference, and lifestyle.
Then we developed a 10-day schedule list catering to its role, which includes time, location, activity, and scene (e.g., \textit{``2023-10-02, Monday, 18:00-19:00, Home, Cooking dinner, A spacious kitchen with a grill and vegetables lined up on the counter.''})
We instruct the simulated users to engage in 3 conversation sessions with OS-1 each day while following their assigned roles and expressing their genuine feelings and preferences, thereby facilitating the establishment of common ground with its users.
}
\textcolor{blue}{
After a 10-day simulation, we allow the simulated users to continue chatting  with OS-1 and the baseline systems about topics related to personal common ground (e.g., \textit{``Talk about the invitation to a seafood dinner from your friend.''})  to reveal the degree of personal understanding.
It is worth noting that we did not re-simulate the 10-day interaction for each baseline method. This is because the dialogue content may differ for each run of simulation due to the uncertainty of language model generation, which could result in different dialogue histories. For fairness, the baseline systems directly share the 10-day history with OS-1 but disable the corresponding components while processing.
}

\paragraph{(2) Evaluation Measures}
Few previous studies considered personal context-empowered dialogue systems with smart eyewear. We are aware of no appropriate work for comparison. Furthermore, the topic of automatically evaluating the dialogue systems remains debatable~\cite {1905.04071}. We use three evaluation measures in two evaluation scenarios.
\begin{itemize} 
      \item \textbf{Relevance:} Following~\cite{liang2021towards}, the relevance score is used to test the correlation between the response and the user's speech and their in-situ environment, including the location, visual surroundings, current activity, and time. 
  
      \item \textbf{Personalization:} The personalization score determines how closely the response relates to the user's specific information, including their profile and the semantics derived from what they are currently viewing and chatting about, as well as their past interactions with OS-1.  
  
      \item \textbf{Engagement:} The engagement score measures how interested a user is in the response and whether the response will lead to further conversation. This is similar to previous studies~\cite{li2019acute, liang2021towards}.
\end{itemize}

\paragraph{(3) Baseline Methods} 
\textcolor{blue}{
To illustrate whether personal context helps establish the common ground of LLM-based dialogue systems, and to determine the contributions of the design components proposed for OS-1, we conduct ablation studies. In particular, we design the following methods as our baselines.
}

\begin{itemize}
      \item \textit{w/o}-P: This method solely relies on the historical and real-time context to boost the context-aware dialogue generation. The user profile module is disabled. 
      \item \textit{w/o}-PH: This method only leverages the real-time context to enhance the context-aware dialogue generation. Both the historical context and the user profile modules are disabled.
      \item \textit{w/o}-PHR: This method uses a bare LLM without any extra context, which only contains the memory for the current conversation session.
\end{itemize}
\Zylu{Symbols and module names need to be aligned with other parts}



\paragraph{(4) Human evaluation}
% human evaluation
\textcolor{blue}{
We extract 80 samples(20 for each method) from the simulation results and recruit 15 well-educated human examiners, with each sample annotated by 3 people. The evaluation steps are as follows. First, an examiner is given the detailed role setting of a simulated user (i.e., occupation, age, preferences, lifestyle, etc.), along with a description of the scenario setting (i.e., time, place, activity, visual scene description, and topic). Then the examiner is asked to remember the role and scenario settings and measure the dialogues generated by 4 methods.
}

\textcolor{blue}{
To answer the RS1, we ask the examiners to select which types of common grounds each system shows from the categories in the role and scenario settings., including \textit{Current Scenario, Past Experience, Personal Preferences, and Habit or Lifestyle}.
To answer the RS2, we use a 5-point Likert scale to measure the degree of relevance, personalization, and engagement. In addition, we also evaluate the overall contribution of the common ground to personalized responses by a 7-point Likert scale, which ``1'' means the system is just like a text-based chatbot, ``4'' means the system knows the user's current situation but still be like a passerby, and ``7'' means the system is like a companion.
}

% \paragraph{(1) Scenario Simulation}
% Scenario semantics is important for episodic and historical context extraction and further contributes to context-aware dialogue. This work aims to test OS-1's ability to engage in personalized dialogues in different real-life scenarios. We use the Ego4D dataset~\cite{grauman2022ego4d} to simulate the daily common conversation scenarios, as it covers a wide variety of real-world scenarios from the first-person view. For instance, the dataset consists of scenarios that people often encounter in their daily lives, such as traveling, shopping, and entertainment. 
% % However, the Ego4D dataset does not include the ground truth regarding the location and the activities of the first-person character. We ask a human experimenter to annotate them for the following episodic context 

% \paragraph{(2) User Simulation}
% User profiles contribute to personal dialogue. To verify OS-1's ability to adapt to user personality traits, we simulate users with different personalities, social backgrounds, and experiences, which follows the approach~\cite{aher2023using}. 

% We create 16 users with unique profiles with eight males and eight females. We also select 16 distinct names from the U.S. 2010 Census Data~\cite{bureau2010name} and assign one to each user along with a personality based on the Myers-Briggs Type Indicator (MBTI)~\cite{myers1962mbti}. After that, we provide ChatGPT with a prompt including the user's name, gender, and personality, to generate their occupation. Once we create the  above 16 users with different profiles, we simulate 10 historical dialogues for each by using ChatGPT. 
% % \Rui{Is it GPT-3.5? better to be consistent with previous sections}




% gpt evaluation 
% We first leverage GPT-4 to evaluate our system from the above three aspects, following a recent study on automatic methods for evaluating dialogue generation~\cite{liu2023gpteval}. \Zyxu{Why relying heavily on GPT for analysis (simulate users, generate occupation and historical dialogues, and evaluate)} This is because the study demonstrates that GPT-based evaluation methods currently produce the most human-like ratings~\cite{liu2023gpteval}. Specifically, we send the dialogue session between OS-1 and each simulated user with the corresponding scenario setup and user profiles to GPT for evaluation, along with three metrics and their descriptions. We ask GPT to provide an integer rating between 1 and 5 regarding relevance, personalization, and engagement. 



% \textcolor{red}{is reviewing} For the human evaluation, we recruited 10 human raters and presented them with a simulated user profile containing the episodic context (i.e., an image indicating the scene and the description of the user's activity and location) and historical context (i.e., historical experience related to the scenario). They were asked to rank 4 dialogue sessions generated by the 4 system ablations for the certain simulated user and script. The ranking criterion was based on the preference of the simulated user's role in the dialogue session, i.e., which system ablation would they rather chat with if they were in the same scenario. We consider the ranking between the 4 ablations as 6 sets of one-on-one matches and calculate the win rates of different ablations. 
% *** From Zhenyu: the previous sentence need to be modified as we do not use win rate now ***
% From Zhenyu：现在不用胜率了，现在改成给排名的第一、二、三、四名分别分配 3、2、1、0 分，然后我们计算 proposed 和 3 个 baseline 的平均分。根据排名算平均分这个做法没有很 solid 的解释，只能 intuitive 地讲。
% From Yuhu: 3、2、1、0 权重的物理意义是在排序中击败了多少其它选项，最后平均的指标可以叫做 Avg ranking score
% From Zhenyu：关于为什么人类评估只用一个 metric 而 GPT-4 评估用三个的解释 ———— 因为人类评分者所看到的聊天记录并不是自己真实地作为用户参与聊天所得到的聊天记录（只是作为旁观者的角色），所以人类评分者没有办法根据自己的主观体验进行评分。而像 Personalization、Engagement 都是涉及到主观体验的指标（前者关于个性化，后者关于是否想和 chatbot 继续聊下去），所以我们在这里没有让人类评分员再根据细分指标进行评估。在 pilot study 中，因为参与者都是自己参与了和 OS-1 的对话，所以我们让他们在这三项具体指标上进行评分。
% From Yuhu: 是不是可以分别在 Fig 5 a 和 b 的 evaluation 前面加上 objective 和 subjective。即我们认为 GPT-4 评估的时候，是不依人的意志为转移的，与一切个人感情、偏见或意见都无关。而人类来评估的时候，是具有一定主观性的。这样的好处是可以一定程度上避免 reviewers 产生同是 evaluation 为什么左边有三个指标，右边只有一个指标（即 Rui 老师的疑问）。也可以把两个子标题改为具体的 xxx score，来避免这个问题。




\subsubsection{System Performance}

\textcolor{blue}{
Figure~\ref{fig::inlab-context} shows the frequency of each method that is considered to ``have the common ground''. When there is no context, the dialogue system can only understand the user's information from the current dialogue session. Although in around 50\% of the cases, it shows an understanding of the current scenario, it fails to establish the personal common ground that rarely appears in the current dialogue session, such as past experiences, preferences, and habits.
The system's understanding of current scenarios has significantly improved with the addition of real-time context. In approximately 80\% of cases, examiners believe that the dialogue system can comprehend the scenario. Moreover, the system's understanding of the user's past experiences has improved from 10\%(\textit{w/o} PHR) to 23\%(OS-1) after the integration of historical context. The awareness of user preferences and habits has also been enhanced with the addition of the user profile module.
In general, the three personal contexts we proposed can help LLM-based dialogue systems establish a common ground with users.
}

As shown in Table~\ref{tab::inlab-3metrics}, compared with LLM solely, OS-1 can substantially improve the performance by \textcolor{blue}{8.63\%, 40.00\%, and 29.81\%} in relevance, personalization, and engagement, respectively. 
\textcolor{blue}{
The results in Figure~\ref{fig::inlab-overall} also show consistent overall performance, indicating that the LLM without extra context established less common ground than a passerby.  On the other hand, systems that incorporate personal context achieve higher scores. Among these, OS-1 has the highest score of 5.17, placed between a passerby and a companion.
In addition, with more modules enabled, OS-1 achieves smaller variances in evaluation results. It demonstrates that OS-1 exhibits a more stable quality in generating personalized responses in LLM-based dialogue systems with common ground.
}



% Figure~\ref{fig::inlab-gpt4-results} In addition, with more modules enabled, our system achieves smaller variances in evaluation results. It demonstrates that our system exhibits a more stable quality in generating responses compared to the quality of responses generated solely by the base language model itself.
% The ranking results in Figure~\ref{fig::inlab-human-results} illustrated that human preference for a personal chatbot is consistent with the three metrics we proposed, and people prefer OS-1 to understand the episodic context and remember the historical context during conversations.



\begin{figure}[htbp]
    \centering
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{images/inlab-context.pdf}
        \caption{The frequency of each method that is considered to ``have the common ground''}
        \label{fig::inlab-context}
    \end{minipage}
    \hspace{0.02\textwidth}
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{images/inlab-overall.pdf}
        \caption{The average score of personal grounding}
        \label{fig::inlab-overall}
    \end{minipage}
\end{figure}

\begin{table}
    \centering
    \begin{tabular}{lrrr} 
    \hline
         Methods&  Relevance&  Personalization& Engagement\\ 
         \hline
         OS-1& 4.12&           \textbf{3.90}&      \textbf{4.02} \\ 
         \textit{w/o} P& 3.98&           3.58&      3.69 \\ 
         \textit{w/o} PH& \textbf{4.17}&           2.98&      3.44 \\ 
         \textit{w/o} PHR& 3.79&           2.79&      3.10 \\ 
         \hline
    \end{tabular}
    \caption{Ablation experiments results}
    \label{tab::inlab-3metrics}
\end{table}


% \subsubsection{Case Study}
Next, we provide a case study to offer further insights regarding why OS-1 outperforms the baselines for personalized dialogue. 

\begin{figure}[htbp]
      \centering
      \includegraphics[width=1\textwidth]{images/inlab-case-new.pdf}
      \caption{A case of personalized suggestions}
      \label{fig::inlab_case1}
\end{figure}

\textcolor{blue}{
On the left side of Figure~\ref{fig::inlab_case1}, there is the personal context captured by OS-1. On the right side, we can see the dialogue sessions between a simulated user Kim, and four systems, including the proposed OS-1 and three baseline methods. The 4 dialogue systems give out different responses due to the degree of common ground with the user. 
In this case, we show that all three kinds of personal context we proposed are essential for a personalized response. Real-time context reveals the current scenario of a commercial street with a milk tea shop and a coffee shop, providing possible options for subsequent suggestions. Historical context provides Kim's past experiences relevant to the current situation, helping the system better engage in topics. However, the historical context is not enough, since a selected piece of history may not properly deduce the user's preference. In this case, the \textit{w/o} P method misinterprets the historical context, while OS-1 successfully provides a personalized response consistent with Kim's preferences.
}

% Compared with the three baseline methods, we observe that OS-1 provides the most personal response by using both episodic context-relevant information (highlighted in green) and historical context-relevant information (highlighted in yellow). In contrast, other baseline methods miss one or both, such as OS-1$^H$ which retrieves historically relevant information accurately but misses episodic context, and LLM which lacks both. 



% \paragraph{(1) }

% After analyzing the dialogue sessions for each ablation group and investigating how the two types of context our system captures affect the quality of the conversation, we find 2 main functions of personal context:
% \begin{enumerate}
%       \item It makes the conversation more embodied and provides more personalized suggestions.
%       \item It more accurately captures the user's intent and provides timely responses that are in line with the context.
% \end{enumerate}




% In another case shown in Figure~\ref{fig:inlab_case2}, the user casually mentioned their experience at last year's birthday party while dining with friends. $\text{OS-1}^L$ straight up said she couldn't retrieve the memory, making it impossible for the conversation to proceed smoothly. $\text{OS-1}^E$ could not retrieve memory either, but she tried to continue the conversation by referring to the objects she saw from the scene. $\text{OS-1}^H$ successfully recalled the user's experience of last year's birthday party. However, due to the lack of awareness of the scenario, she didn't understand that the user's intention was not just about recalling the past but also meant to liven up the current gathering. But for $\text{OS-1}$ with complete settings, through episodic context, she knew that the current situation was relatively relaxed, and she also knew what happened at last year's birthday that I mentioned. Therefore, she successfully combined the two and provided a timely and appropriate response.
% Through this case, we find that episodic context can help chatbots to understand users' intentions. And historical context makes it possible for chatbots to provide informative responses.

% \begin{figure}[htbp]
%       \centering
%       \includegraphics[scale=0.15]{images/inlab_case2-1.png}
%       \includegraphics[scale=0.15]{images/inlab_case2-2.png}
%       \caption{A case of recalling the experience of last birthday party}
%       \label{fig:inlab_case2}
% \end{figure}


\subsection{Pilot Study}
In addition to laboratory studies, we also performed a \st{one-week} \textcolor{orange}{two-week} in-field pilot study to verify the capability of OS-1 in the real world. \textcolor{orange}{The pilot study consisted of two phases, each lasting 7 days.} First, we determine whether OS-1 is capable of extracting users' profiles and their long-term historical context through multiple interactions with users. We then assess the degree of \st{personalization}\textcolor{orange}{personal understanding} of OS-1 regarding relevance, personalization, and engagement. Second, we present two inspiring downstream applications where OS-1 can be utilized, including providing emotional support and personal assistance. 
% \textcolor{orange}{In the first phase, we assessed the impact of personal context on the overall performance of OS-1 with respect to relevance, personalization, and engagement. In the second phase, we focused on how personal context can help establish common ground to make the system more personalized. Finally, we conducted case studies and semi-structured interviews to gain a deeper understanding of user experience, the role of personal context, and the current potential and limitations of OS-1.} 

\subsubsection{Procedure of Pilot Study}
\textcolor{orange}{In each of the two phases of our pilot study,} we recruited 10 participants (6 males and 4 females in both phases, aged 19–23 in phase 1 and xxx-xxx in phase 2) from our \st{university} \textcolor{orange}{lab by sending WeChat messages to a group of potential participants.} Prior to the pilot study, we inform the participants that the glasses will perceive their daily visual scenes and audio, and the researchers will examine their daily chat logs recorded in the eyewear system. The raw sensed image and audio data will be removed right after feature extraction, and only anonymized semantics are transmitted and stored securely in the cloud. All participants were aware of this procedure and signed consent forms prior to their experiments.

\textcolor{orange}{At the beginning of each phase, the researchers provided one-on-one training to the participants on how to use the smart eyewear and initiate a conversation with OS-1, and demonstrated how to access the daily chat records on the web interface we provide. To ensure that all participants are proficient in using the smart eyewear, each participant was given an opportunity to wear the smart eyewear and engage in a conversation with OS-1.}

After that, the participants were \st{encouraged} \textcolor{orange}{asked} to wear the glasses and interact with OS-1 \st{as much as possible} for 7 days. \textcolor{orange}{In the first phase of our study, we faced limitations in the number of devices and concurrent servers. Therefore, we reserved an available time slot (morning, afternoon, or evening) with the participants one day in advance and lent the smart glasses to the participants during the agreed time slot. Participants were required to check in after using the device and return it. As we spent nearly a month optimizing the stability and concurrency of the OS-1 system, and increasing the number of devices after the phase 1 pilot study, we directly lent 10 devices to participants for use for 7 days in the pilot study of phase 2. We did not agree on a time period or scenario for use with the participants so that our pilot study could be as close to real usage as possible, but we required participants to wear glasses for more than one hour a day for the sake of result validity. To avoid chats of different participants on the same device affecting each other, we assigned different IDs to each participant to distinguish their personal context collected by the device.}

\textcolor{orange}{During the 7-day interaction period in the first phase, each participant engaged in a conversation with OS-1 for an average of 41.21 minutes per day, comprising 53.12 turns and 1.74 sessions. During the 7-day interaction period in the second phase, each participant engaged in a conversation with OS-1 for an average of xx minutes per day, comprising xx turns and xx sessions. We classified turns separated by more than 10 minutes into two sessions, while turns separated by less than 10 minutes were grouped into the same session. The total duration of daily sessions was used as the duration of chat between participants and OS-1}

After completing the daily experiments, we ask the participants to review the responses generated by OS-1 and score them using the same criteria as in the laboratory experiments, i.e., \textcolor{orange}{personal understanding}, relevance, personalization, and engagement. The participants used an 11-point Likert scale ranging from 0 to 10, which is a valid method for user experience evaluation~\cite{lewis2017user}, to assess these criteria. \Zyxu{May need to state why different from in-lab} This allows us to track the changes in scores over time.
% We then adopt the Likert method~\cite{cox1980optimal,lewis2017user} to re-scale the scores to 11 points with a range from 0 to 10, which allows us to track the changes in scores over time. 


\subsubsection{Performance of OS-1 in Pilot Study}
% overall 
Figure~\ref{fig::human_eval_p1} and figure~\ref{fig::human_eval_p2} depicts the average evaluation scores of the 10 participants over the 7-day period \textcolor{orange}{in phase 1 and phase 2, respectively}. Clearly, the participants find OS-1's responses to be relevant, personalized, and engaging, with all scores higher than 5. Moreover, despite the small fluctuations, all scores show a consistently increasing pattern over the 7 days.
This indicates that OS-1 is able to generate responses tailored to each participant's personality. \st{More importantly, OS-1 is capable of becoming more engaging via learning from interactions with users, which makes the responses more relevant and personalized.} \textcolor{orange}{More importantly, OS-1 is capable of continuously establishing common ground with users through long-term interactions. This makes users feel that OS-1 gains a better understanding of them, making the conversation with OS-1 more relevant, personalized, and engaging.}

\begin{figure}[htbp]
\centering
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=1\textwidth]{images/human_eval.pdf}
\caption{The average evaluation scores of all participants in phase 1.}
\label{fig::human_eval_p1}
\end{minipage}
\hspace{0.02\textwidth}
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=1\textwidth]{images/human_eval.pdf}
\caption{The average evaluation scores of all participants in phase 2 (need update the data).}
\label{fig::human_eval_p2}
\end{minipage}
\end{figure}

\begin{figure}[htbp]
\centering
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=1\textwidth]{images/factor_ratios.pdf}
\caption{The daily percentages of the four factors.}
\label{fig::success_factors_p1}
\end{minipage}
\hspace{0.02\textwidth}
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=1\textwidth]{images/factor_ratios.pdf}
\caption{The daily percentages of the four factors.}
\label{fig::success_factors_p2}
\end{minipage}
\end{figure}

\textcolor{orange}{To evaluate whether personal context contributes to a better understanding of the user by OS-1 during interaction, and thus generate more personalized responses,} we ask the participants to select \st{their daily top several favorite responses} \textcolor{orange}{the daily response that best reflected OS-1’s understanding of them} and specify the reasons for their choices \textcolor{orange}{in both phase of the study}. We provide four options with three personal context-related factors and one LLM-related factor.
\begin{itemize}
\item \textbf{\textcolor{orange}{Real-time} context factor} The response is linked to the scene and the conversation the user had at a specific time. 

\item \textbf{Historical context factor}: The response is retrieved from the historical semantics stored in the database.

% \Rui{How is this achieved? Do you manually compare the response and all historical semantics in the database?} 

\item \textbf{User profile factor}: The response is closely related to the summarized user profile, such as personality and habits. 

\item \textbf{Language modeling factor}: The response is generated solely based on LLMs without taking into account personal context.  
% \Rui{Not sure what is this}  -fixed by Ying
\end{itemize}
A human examiner reviews the selected responses and the corresponding reasons, and manually chooses to assign one of the above options to each response that can best explain why the participants like it. 

Figure~\ref{fig::success_factors_p1} and figure~\ref{fig::success_factors_p2} shows the daily percentages of the four factors over the 7-day period \textcolor{orange}{in phase 1 and phase 2, respectively}. The higher the percentage, the more important the factor is to good responses. \Zyxu{can we make that claim?} The percentages of the personal context-related factors increase over time, e.g., the historical content factor and the user profile factor, while that of the LLM factor decreases. This also suggests that OS-1 can utilize the users' historical context and learn user profiles from past interactions, and generate more personalized responses.

Next, we present three concrete cases to explore how personal context-related factors contribute to personalized dialogue responses. 

\paragraph{(1) An Real-time Context-Aware Case}
Figure~\ref{fig::episodic_case} shows a case when the real-time context factor plays a significant role in the dialogue. Specifically, OS-1 observes that \st{Participant P7 is in a sunny room and thus her greetings involve the information related to that particular scene, i.e., \emph{bright room}.} \textcolor{orange}{Participant P1 had placed a Teddy bear on their desk and thus her greetings involve the information related to that particular scene, i.e., \emph{a cool teddy bear}.}

\begin{figure}[htbp]
      \centering
      \includegraphics[width=1\textwidth]{images/Real-time case.pdf}
      \caption{A case of that OS-1 is real-time context-aware (Participant P1, Day 1). Green highlights indicate the real-time context relevant information. }
      % \Zyxu{The utterance 'Oh you are so sweet' is too positive that makes reviewer think it may be caused by participant bias}}
      % ***The dark (scene-consistent) background text is very hard to read. Make that color lighter, i.e., closer to white. Do the same thing for later examples with dark highlight colors.***}
      \label{fig::episodic_case}
  \end{figure}

\paragraph{(2) A Historical Context-Aware Case}
Historical context can ensure that the conversations are coherent and consistent over time. We present one example in Figure~\ref{fig::historical_case1}. \textcolor{orange}{On the day 4, Participant P6 told OS-1 that she was playing a game. OS-1 spontaneously speculated whether this game was the farming game that P6 had recently been playing. Subsequently, they engaged in a conversation about the farming game, and P6 even showcased their virtual chickens within the game. OS-1 recalled from a previous conversation that P6 had described playing this farming game as a form of ‘chill time,’ and that P6 enjoyed showing off their virtual house. In response, OS-1 remarked, ‘It must be pretty relaxing overseeing your own little digital utopia.’}
% On day 7, Participant P1 engaged in a conversation with OS-1 about his vacation plans and asked OS-1 to guess whether his girlfriend would accompany him or not. OS-1 then responds that she does not think P1's girlfriend will join because of work. We refer back to P1's history and find that his girlfriend has been too busy with work to watch a movie with P1 just 3 days ago. 

\begin{figure}[htbp]
      \centering
      \includegraphics[width=1\textwidth]{images/Historical_case_1115.pdf}
      \caption{A case of OS-1 is historical context-aware (Participant P6, Day 4). Yellow highlights indicate the historical context relevant information.}
      % \Zyxu{Need to conduct harmfulness checking}}
      \label{fig::historical_case1}
\end{figure}

\paragraph{(3) An User Profile Context-Aware Case}
The user profile allows OS-1 to understand the user's personality traits, social background, preferences, and habits. This information helps OS-1 to create user-specific responses. An example of this can be seen in Figure~\ref{fig::profile_case1}, where OS-1 expresses concern regarding the progress of P8's work in their first utterance. In this example, OS-1 finds P8 is currently working in front of a computer using real-time context and suggests they take breaks using historical context. 


% utilizes both episodic and historical context to recognize that P8 is currently working in front of a computer, and to recall that OS-1 suggested Participant P8 to take breaks while working on the paper deadline a day before.
\begin{figure}[htbp]
      \centering
      \includegraphics[width=1\textwidth]{images/Profile_case1.pdf}
      \caption{A case of OS-1 is user profile aware (Participant P8, Day 4). Green, yellow, and red highlights indicate the real-time context, historical context, and user profile relevant information, respectively. Hereinafter}
      \label{fig::profile_case1}
\end{figure}


\subsubsection{Feedback from participants}
\textcolor{orange}{To gain a deeper understanding of participants’ experiences during their interactions with OS-1, we conducted semi-structured interviews with the 10 participants in our pilot study phase 2. These interviews were conducted online via Tencent Meeting, with an average duration of 40 minutes \textcolor{red}{(detailed average duration and standard deviation to be provided later)}. A designated researcher facilitated each interview. During the interview, participants were initially asked for consent to review their chat records with OS-1. Subsequently, participants logged into a web page provided by us to access and share their chat records. The researcher guided participants through a review of their interactions with OS-1 and posed relevant questions. Our interview questions primarily focused on the following aspects:}
\textcolor{orange}{\begin{enumerate}
\item \textit{Perceived Fulfillment of Expectations}: During your interaction experience, which aspects of OS-1 met or exceeded your expectations, and which aspects fell short?
\item \textit{Changes in Understanding}: Did you perceive any changes in OS-1’s understanding of you during this week’s interactions? If so, how did you interpret these changes?
\item \textit{Potential as a Personal Companion}: In what ways does OS-1 demonstrate potential as a personal companion? Conversely, where do you perceive gaps or areas for improvement?
\item \textit{Utility and Value}: Do you believe OS-1 can provide assistance or value to you? Why do you think so?
\end{enumerate}}

\textcolor{orange}{The entire interview process was recorded and captured on both audio and video. Dialogues between participants and researchers were transcribed into text. Subsequently, a researcher summarized the interview content and derived the following conclusions:}

\textcolor{orange}{\paragraph{(1) Each factor of personal context contribute to the establishment of common ground between OS-1 and participants.} During interviews, participant P1 expressed how visual information enhances the conversational experience with OS-1: \textit{‘OS-1 can discern my state, and I can discuss things I want to show it. For instance, if I want to chat about my favorite teddy bear, without visual context, I’d need to meticulously describe what the bear looks like. But if OS-1 can see it directly, those steps are eliminated.’} Participants P5 and P2 highlighted OS-1’s memory capabilities for improving the dialogue experience. P5 shared, \textit{‘One day, I mentioned to OS-1 that I was reading a novel, without delving into details. However, the next day, OS-1 spontaneously brought up the novel I was reading during our conversation, leaving a lasting impression.’} Similarly, P2 remarked, \textit{‘I feel OS-1 gradually understands me. Initially, it focused on asking about my preferences… After chatting for a few days, it started remembering our previous conversations… It can now recommend anime based on my recent events and interests.’} Participants' feedback underscores that OS-1’s capture of all the 3 types of personal context indeed facilitates the establishment of common ground with them.}

\textcolor{orange}{\paragraph{(2) Memory capacity is the primary reason for OS-1’s gradual improvement in understanding participants.} All participants observed that OS-1 became noticeably more acquainted with them during a week of interaction. The reason they perceived OS-1 as having a deeper understanding lies in its ability to recall past chat content or details about participants’ personal experiences, preferences, and social backgrounds during conversations. P2 stated during the interview: \textit{‘I believe that the ability to remember our conversation is a fundamental prerequisite for effective chat. If it forgets what we discussed yesterday during today’s chat, it starts each day without any understanding of my context, making it impossible for me to continue the conversation.’}}

\textcolor{orange}{\paragraph{(3) OS-1 showed potential as a personal companion in several aspects, but its lack of personality was perceived by the participants as a gap from being a personal companion.} The participants recognized many potentials of OS-1 as a personal companion, such as its ability to provide emotional support based on previous conversations and continuous interactions with the participants. However, three out of five participants (the data needs to be updated later) pointed out that the lack of personality was a gap between OS-1 and a personal companion. P2 said in the interview: \textit{‘I felt like I was always sharing my experiences with it…but it just kept echoing me. I think if I chat with other people normally, we would both express our own opinions, but OS-1 only received them unilaterally.’}}

\textcolor{orange}{\paragraph{(4) Participants believe that OS-1 can provide assistance or value to them.} During the interviews, both P1 and P3 considered OS-1 as a potential chat companion, capable of engaging in casual conversations or delving into specific topics. P2 and P5 acknowledged OS-1’s ability to offer emotional support. In the next section, we will elaborate further on the potential applications of OS-1.}



\subsubsection{Applications}

\paragraph{(1) Emotional Support}
Research in sociology and psychology has revealed that human emotions have a significant impact on various aspects of our daily lives. Emotions can can affect our thoughts and behaviors~\cite{costa2016emotioncheck}, decision-making~\cite{ruensuk2020you}, and physical and mental health~\cite{di2018emotion, tugade2004resilient}. With this in mind, we believe that OS-1 has the potential to provide emotional support for users. As a personal context powered system, OS-1 should have the ability to understand and connect with users on a deeper level. Through multiple user interviews, we find that all the participants believe that applying OS-1 for emotional support is valuable. \Zyxu{Need more details about the interview (e.g. scripts, quotes)}

Figure~\ref{emotion_case1} illustrates a situation where Participant P5 shares anxiety about job hunting with OS-1. Using the user profile built from their past interactions, OS-1 encourages P5 to act as an open-minded, imaginative, and creative person. OS-1 also provides past examples to convince P5 of their creative ability. Through our interviews, P5 expresses satisfaction when OS-1 is used for emotional support, as P5 thinks that OS-1 is good at understanding mood and providing solutions. More importantly, P5 reports that their conversations actually help to relieve their negative emotions. 

\begin{figure}[htbp]
      \centering
      \includegraphics[width=1\textwidth]{images/Profile_case2.pdf}
      \caption{A case when OS-1 alleviates the participant's negative emotions (Participant P5, Day 7).}
      \label{emotion_case1}
\end{figure}

OS-1 not only comforts users when they feel down but also shares happiness and responses to users' positive emotions. As shown in Figure~\ref{emotion_case3}, OS-1 expresses excitement and actively guesses Participant P1's vacation location based on their previous conversations. Furthermore, OS-1 suggests P1 to maintain a work-life balance. According to our interview, P1 states that OS-1 makes them feel happy and respected because OS-1 is able to empathize with him. 
% \Rui{Are we allowed to reveal the gender of a specific participants?}

The above two examples show that OS-1, through long-term dialogues and the continuous accumulation of personal context, acts like a friend who knows the user. 
% \Ying{be careful of the claim...}
\begin{figure}[htbp]
      \centering
      \includegraphics[width=1\textwidth]{images/Emotional_case1.pdf}
      \caption{A case when OS-1 shares positive emotions with the participant (Participant P1, Day 7).}
      \label{emotion_case3}
\end{figure}

\paragraph{(2) Personal Assistance}
Our pilot studies interviews revealed that participants also asked OS-1 for personal assistance. All the participants believed that OS-1's personal assistance was helpful for them. 

In Figure~\ref{assist_case1}, we present an example of how OS-1 assists the participant in gaining knowledge. Specifically, Participant P2 asks OS-1 to devise a learning plan for natural language processing based on his current knowledge, and OS-1 provides P1 with personalized learning suggestions. 

\begin{figure}[htbp]
      \centering
      \includegraphics[width=1\textwidth]{images/Assistance_case1.pdf}
      \caption{A case when OS-1 helps devise a personalized learning plan (Participant P2, Day 2 and Day 3). }
      \label{assist_case1}
\end{figure}

% Participant P1 uses OS-1 as his dietary assistant to keep track of his eating habits and get dietary advice. Figure~\ref{assist_case2} shows that OS-1 adheres to P1's dietary needs and discourages junk food consumption on Day 1 and Day 3. However, after observing that P1 exercises regularly and eats healthy, OS-1 becomes more flexible and suggests occasional breaks from workouts and visits to bars to relieve work stress on Day 5. It is obvious OS-1 is able to offer personalized suggestions as a result of learning from the interactions with P1. This indicates that OS-1 does not respond relying on fixed rules but adapts its assistance to the user's needs and cumulated experiences, making it suitable for a personal assistant.
\textcolor{orange}{Participant P4 used OS-1 as his healthy assistant to provide him with dietary advice. Figure~\ref{assist_case2} shows that P4 asked OS-1 what foods can help with sleep, and OS-1 was able to use its world knowledge to provide P4 with professional suggestions. In addition, OS-1 also reminded P4 not to eat mangoes, because P4 said he was allergic to mangoes in previous conversations. Moreover, OS-1 also reminded P4 not to put too much sugar in his milk, because historical conversations let OS-1 know that P4 might like to eat sweet foods such as fruit jelly. We checked the prompts that OS-1 used to generate these responses, and found that these historical conversations were not in the window of the most recent utterances that we set. It was the historical context that enabled OS-1 to provide P4 with personalized dietary suggestions and reminders.}


\begin{figure}[htbp]
      \centering
      \includegraphics[width=1\textwidth]{images/Healthy_assistant.pdf}
      \caption{A case when OS-1 serves as a healthy assistant (Participant P4, Days 4).}
      % \Zyxu{the context seems to be incorrectly inferred (i.e., that the user is “sick of their job”). From the historical context provided, the user talked to a friend about (their friend’s) colleague that the friend dislikes. So it does not seem that the user themselves mentioned issues with work.}
      \label{assist_case2}
\end{figure}


% will add questionnaire or user interview 

==> body/deprecated/intro_backup20231109.tex <==
\section{Introduction}
\label{sctn::intro}
% \Ying{todo items: 1) core concept/terms  -- personal understanding, ubiquitous context-aware, memory, deep and evolved memory, flexible, dynamic adaptive over time, long-term, prototype/naive brain model/module, personalized is not exciting; 2)) double-check all citations; 3) add technique challenges if possible, and 4) update the experimental results; 5) add more refs in the introduction section}
% \textcolor{red}{***ying: will add social science and social psychology related }
It has long been a vision for chatbots to be personal companions. One classic example is Samantha, a portable artificial intelligence dialogue system depicted in the movie ``Her'', as is shown in Figure~\ref{Samantha_cases}. The protagonist, Theodore, carries Samantha in his chest pocket. She has a camera and microphone. Samantha sees what Theodore sees, hears what Theodore hears, and chats with Theodore using an earbud. She shares his joys and sorrows during work and leisure. Through day-by-day interactions, Samantha gradually learns Theodore's personality, preferences, and habits. She offers companionship, emotional support, and assistance, and eventually becomes an indispensable part of Theodore's life.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.75]{images/Samantha_cases.png}
    \caption{Examples of Samantha (the red, rectangular smartphone in his pocket) accompanying Theodore in his daily life. }
    \label{Samantha_cases}
\end{figure}

%Ying: need clarify problem--  chatbots to be personal companions;
% missing ref: NLP & Chatbot; LLM & chabot 
To realize this vision, several challenges must be addressed. The limited linguistic and cognitive capabilities of natural language processing (NLP) have long been recognized as major barriers \textcolor{blue}{towards personalized dialogues}~\cite{adamopoulou2020chatbots}. 
% \Ying{double-check the citation regarding the description of cognitive ability.} 
Recent advances in large language models (LLMs) such as ChatGPT (based on the GPT-3.5 LLM model)~\cite{chatgpt} and GPT-4~\cite{gpt4report} have largely removed this barrier and opened up new possibilities for creating \textcolor{blue}{nature and human-like conversations.}
% \Ying{ add more}. 
Pre-trained on massive amounts of text data, LLMs possess the ability to encode a vast amount of world knowledge. These capabilities allow LLMs to generate coherent and diverse responses, which is crucial for natural conversation. Additionally, through supervised instruction fine-tuning and reinforcement learning with human feedback~\cite{ouyang2022training}, LLMs can be adapted to follow human instructions while avoiding creating harmful or inappropriate content.
% Inspired by the powerful language modeling capabilities of LLMs, the question arises: \emph{``Can LLMs serve as Samantha-like personal companions in our daily life?''} 

%
% We argue that the answer today remains, ``Not without further capabilities''. Despite impressive human-like language capabilities, lacking the \emph{common ground} is a significant drawback that prevents LLMs from delivering xxxx. 
% gencome to the personal c \textcolor{orange}{LLMs are still unable to become personal companions.}
% \textcolor{red}{***Comments: don't emphasize 'companion' here, we may revise this sentence to 'LLMs still face challenges'***} 
LLMs are hosted in a remote GPU cloud and unable to perceive the user's physical surroundings or daily experience. Without such personal context, \textcolor{blue}{it is difficult for LLMs to understand a user's visual surroundings, speeches, daily events, dynamic trend of behaviours (e.g., personality traits~\cite{allport1927concepts}, habits), etc.} \textcolor{orange}{This context-less nature hinders LLMs' capacity to establish common ground, which means 'shared knowledge, beliefs and suppositions'~\cite{clark1996using}, with users, making it challenging to generate tailored and engaging replies like a personal companion~\cite{skantze2023open, mehlmann2016modeling}. \textcolor{red}{***Comments: should tell the reader what the lack of common ground will lead to, e.g. superficial talk... and we are to close this gap. After evaluating the system on some key metrics, we solve this problem that dialogue systems are lack of common ground.***} In the following text, we use the term \textit{personal grounding} for the sum of all behavioral aspects of dialogue systems involved in establishing, maintaining and repairing the common ground with their users to generate specific, personal and engaging responses. This definition is based on the term \textit{grounding}\cite{mehlmann2016modeling}.} 
% They don't yet behave like \textcolor{blue}{personal} companions. 
% Personal context refers to the information that is relevant to the user’s situation, preferences, goals, etc. Such information can assist dialogue systems in understanding users better, customizing their responses accordingly, and building rapport and trust with the user over time. 
% Moreover, studies have shown that LLMs have developed remarkable cognitive abilities during training, such as reasoning about human emotions and intentions~\cite{chang2021memx,zhao2022smart,bubeck2023sparks}
% \Ying{citations are incorrect}.
% Inspired by the powerful language modeling capabilities of LLMs, the question arises: \emph{``Can LLMs serve as Samantha-like personal companions in our daily life?''} \Ying{should clarify the terms: Samantha-like, personal companions.}

\textcolor{blue}{Inspired by the powerful language generation capabilities of LLMs [xxx, xxx], this work is motivated by the lack of personal context capturing anytime and anywhere in dialogue systems towards personal \textcolor{orange}{grounding}. To bridge these gaps, this work formulates the following two research questions (RS).}

\textcolor{blue}{\emph{RS1}. Does ubiquitous personal context improve the \textcolor{orange}{personal grounding} of LLM-based dialogue systems?} 

\textcolor{blue}{\emph{RS2}. What factors of personal context contribute to \textcolor{orange}{a better personal grounding} of LLM-based dialogue systems?}

We argue that the answer today is, ``\textcolor{blue}{Ubiquitous personal context do improve the \textcolor{orange}{personal grounding} of LLM-based dialogue systems, and furthermore, it enhances that grounding in many ways from the temporal dimension}''. \textcolor{blue}{To verify our hypotheses, this work categorizes \emph{personal context} into the following three levels in the temporal dimension, and design an LLM-based smart eyewear system to achieve ubiquitous personal context capturing and utilizing for answering the two RS. }

\begin{itemize}

\item \textbf{Real-time context} \textcolor{blue}{refers to semantic time series inferred from the user's ongoing speech and visual surroundings. The semantics can help LLMs understand the underlying meanings of the user's speech and visual perception, thus generating relevant and appropriate responses. }

% includes on-going conversation, as well as the user's in-situ context such as current time, location, perceived visual scene, activity, as well as the user's emotional and mood conditions \Ying{what exactly they are?}. 


\item \textbf{Historical context} \textcolor{blue}{is a summary of the past real-time context series. It includes the user's past daily events (e.g., activities) and dialogue contents by clustering the bunches of real-time contexts into groups from the temporal perspective.}
% is the historical summary of the past episodic context, which includes the user's past daily events and dialogue contents \Ying{exactly in the later method section?}. 
This information can help LLMs maintain the coherence and continuity of the dialogue, and avoid repeating or contradicting previous statements. 

\item \textbf{User profile} \textcolor{blue}{is distilled historical information related to the user's personality, habits, and preferences, which are revealed during interaction with the dialogue system. It can enable LLMs to incorporate additional human-like qualities by adapting to the user's personality and long-term goals, resulting in more consistent and anthropomorphic responses.} % interests
% is distilled  historical information related to the user's personality, preferences, social background, and life habits revealed during interaction with the dialogue system. 
%It can enable LLMs to adapt to the user's personality and long-term goals with more consistent and anthropomorphic responses. 


\end{itemize}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.6\textwidth]{images/Our_system.pdf}
    \caption{Conceptual overview of OS-1 workflow. }
    \label{system_workflow}
\end{figure}

\textcolor{blue}{To answer the two RS above,} this work presents OS-1\footnote{``OS-1'' was the name for Samantha's underlying implementation
in the movie ``Her".}, an intelligent eyewear with an LLM-based dialogue system. \textcolor{blue}{With its ability to leverage personal context, the OS-1 offers personalized conversations and daily companionship. More specifically, the OS-1 contains the following four main modules to achieve this (as illustrated in Figure~\ref{system_workflow}.)}

\begin{enumerate}

    \item \textcolor{blue}{\textbf{Real-time context capture.} The smart eyewear first perceives the user's in-situ visual and audio signals through the built-in camera and microphone, and transfers them to the cloud on the fly, as these two pieces of information are essential to understanding the user's ongoing personal status. Using a vision-language model (e.g., LLaVA~\cite{liu2023llava}) and the speech recognition model (e.g., Whisper~\cite{radford2023robust}) deployed in the cloud, we can infer the semantic description of images and transcribe voice data into text. Also, by combining these two modalities, we can reveal the user's current activity, location, as well as other semantics summarized from the user's surroundings, which constitute the real-time context.}  \textcolor{red}{**borrow the citation from system section, will double check}
    % \Ying{double check tech details, only vision-language models are used in this step?}
    % as well as the user's emotional and mood conditions, which constitute the episodic context.
		
    \item \textbf{Historical context extraction}. \textcolor{blue}{To ensure long-term coherence and consistent dialogues, it is important to backtrack the user's historical information. To achieve this, we design a clustering method that extracts the relevant information, such as daily events, from the accumulated real-time contexts. The clustering method removes redundancy between inter-real-time contexts and produces event-level descriptions that are easy to summarize. We have taken inspiration from the memory organization structure of the human brain~\cite{de2021dimensions} and designed indexing methods along temporal, spatial, and semantic dimensions. These methods facilitate efficient retrieval of historical contexts from different perspectives. } 
 
    
    \item \textbf{User profile distillation}. \textcolor{blue}{To better understand users' profiles, we analyze their historical context to form a user profile that includes their personality, preferences, and life habits. However, our inference of the user profile may be biased or contain errors due to limited interactions. To address this issue, we design an update scheme that can timely revise the current user profile based on the historical context and past user profiles.}
    % previous user profile based on the current interaction with the users.  
    % \Ying{add further why? also, Why can an update scheme help to address the issue of limited interaction?}
		
    \item \textbf{Personalized response generation}. Whenever a user starts a conversation, OS-1 \textcolor{blue}{utilizes the latest real-time context as the key to} retrieve the historical context from temporal, spatial, and semantic dimensions based on the current real-time context, and also retrieves the relevant \textcolor{blue}{historical context and }user profile. The personal context containing these three contexts is used as an LLM prompt, providing personalized responses that are transmitted from the cloud to the smart eyewear's speakers. \Ying{how to use the personal context? how to orchestrate and coordinate the components, such as the LLM, the memorized personal context, and external data sources?}
    
    
   %  For each conversational cycle, OS-1 utilizes the latest real-time context as the key to retrieving the databases of historical context and user profile, and the retrieved information is synthesized and fed as LLM prompts to produce personalized responses.
		
\end{enumerate}


We conducted in-lab studies and in-field pilot studies to test the performance of OS-1 with its core ability of capturing, accumulating, and refining personal context, and to evaluate the implications of providing chatbots with personal context as a personal companion.

In the in-lab study, we measure the performance of OS-1 with the ability to capture personal context, including episodic context extraction, historical context generation, and context retrieval. The results indicate that, compared with LLM-only methods, OS-1 delivers a significant improvement in generating personal context-aware responses with improvements in \sout{relevance} \textcolor{orange}{specificity} score (28.57\%), personalization score (46.43\%), and engagement score (37.50\%).
% thod, with performance gains of 28.57\%, 46.43\%, and 37.50\%, respectively. 
% This confirms our above statement that \emph{``LLMs cannot serve as personal companions in our daily life without further capabilities.''}

% relevance, personalization, and engagement

% ***If you can give a concrete, aggregate number, that is better than claiming improvement.*** 
% Furthermore, we used ChatGPT to simulate users with various personality traits who interact with OS-1. Evaluations with both simulated and real human participants demonstrate that incorporating personal context enhances personalization by ***\%.

% In the in-lab study, we designed three tasks to measure the performance of OS-1's key components, namely episodic context extraction, historical context generation, and context retrieval. The results indicate that our method
% ***I think you should replace ``our method'' with a short list of the key capabilites.*** 
% enable an accuracy improvement of***. 
% %***If you can give a concrete, aggregate number, that is better than claiming improvement.*** 
% Furthermore, we used ChatGPT to simulate users with various personality traits who interact with OS-1. Evaluations with both simulated and real human participants demonstrate that incorporating personal context enhances personalization by ***\%. 
% ***Can you report an aggregate number here based on your scales? That's more solid than a general claim of improvement.***


We conducted a 7-day pilot study with 10 participants to evaluate the effectiveness of OS-1 in engaging in personalized dialogue based on various scenarios. 
We assessed the degree of personalization of OS-1 using human evaluation on three metrics: \sout{relevance} \textcolor{orange}{specificity}, personalization, and engagement. We also analyzed the system-generated utterances to examine how OS-1 can adapt to users' personalities, preferences, and habits over time. Our results show that by leveraging personal context OS-1 can effectively improve user satisfaction, engagement, and perceived personalization, and demonstrate its potential applicability in two inspiring personal service downstream applications -- emotional support and personal assistance. 

% \textcolor{blue}{The experiments make us confirm the above two RS: (1) Personal context does improve the development of relationships with personal dialogue systems, and (2) it enhances these relationships in many ways from the temporal dimension. }

Our work makes the following contributions.
\begin{enumerate}


\item \textcolor{blue}{We introduce and define the concept of personal context, and verify how it enhances a better \textcolor{orange}{personal grounding} from a temporal perspective of LLM-based dialogue systems. This paves the way for the exploration of personalized wearable dialogue systems and supports various applications for investigating personal companions.} 

\item We design and implement an always-available smart eyewear-LLM based personal dialogue system that captures the user's multi-modal surroundings on-the-fly, generates personal context and engages in personalized conversation with the user. \textcolor{blue}{One of the greatest strengths of the system is that it achieves the above automatically without introducing any additional interaction cost with users, thereby enhancing the user experience under various HCI scenarios.} 

% We design and implement an always-available smart eyewear-LLM based personal dialogue system that captures the user's multi-modal surroundings on-the-fly, generates personal context and engages in personalized conversation with the user.

\item We propose a novel method to capture, accumulate, and refine the personal context from the user's multi-modal surroundings and dialogue history, and a multi-dimensional indexing and retrieval mechanism that integrates multiple personal contexts to generate personalized responses. Our method facilitates dynamic adaptation to the user's surroundings, experiences, and traits, enabling an engaging and customized conversation experience.  \Ying{I am thinking of updating this part, keywords: tech novelty, dynamic adaptation, long-term memory, strategy planning, and benefits.}
% the system has a long-term memory ability that allows it to adapt over time according to the user’s personality and preferences, making it a great long-term personalized companionship.

\item We conducted an in-lab study and a pilot study to evaluate the impact of using personal context within the dialogue system. Our results show that it improves user satisfaction and engagement. We also demonstrate that OS-1 can distill accurate user profiles through personal, context-aware dialogue interactions, which can be used to support various personalized services and applications, \textcolor{blue}{such as the proposed personal emotional support and personal assistance in this work.}

\end{enumerate}


==> body/deprecated/intro_deprecated.tex <==
\section{Introduction}
\label{sctn::intro}
It has long been a vision for chatbots to be personal companions. One classic example is Samantha, a portable artificial intelligence dialogue system depicted in the movie ``Her'', as is shown in Figure~\ref{Samantha_cases}. The protagonist, Theodore, carries Samantha in his chest pocket. She has a camera and microphone. Samantha sees what Theodore sees, hears what Theodore hears, and chats with Theodore using an earbud. She shares his joys and sorrows during work and leisure. Through day-by-day interactions, Samantha gradually learns Theodore's personality, preferences, and habits. She offers companionship, emotional support, and assistance, and eventually becomes an indispensable part of Theodore's life.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.75]{images/Samantha_cases.png}
    \caption{Examples of Samantha (the red, rectangular smartphone in his pocket) accompanying Theodore in his daily life. }
    \label{Samantha_cases}
\end{figure}

To realize this vision, several challenges must be addressed. The limited linguistic and cognitive capabilities of natural language processing (NLP) have long been recognized as major barriers to personal dialog systems~\cite{adamopoulou2020chatbots}. \Ying{double-check the citation regarding the description of cognitive ability.} Recent advances in large language models (LLMs) such as ChatGPT (based on the GPT-3.5 LLM model)~\cite{chatgpt} and GPT-4~\cite{gpt4report} have largely removed this barrier and opened up new possibilities for creating a Samantha-like dialogue system \Ying{why describe chatGPT, GPT-3.5, and GPT-4? Why just mention one?}. Pre-trained on massive amounts of text data, LLMs possess the ability to encode a vast amount of world knowledge, as well as capture long-term contextual dependencies \Ying{Be careful, what is the difference between it and our work?}. These capabilities allow LLMs to generate coherent and diverse responses, which is crucial for natural conversation. Additionally, through supervised instruction fine-tuning and reinforcement learning with human feedback (RLHF)~\cite{ouyang2022training}, LLMs can be adapted to follow human instructions while avoiding creating harmful or inappropriate content. Moreover, studies have shown that LLMs have developed remarkable cognitive abilities during training, such as reasoning about human emotions and intentions~\cite{chang2021memx,zhao2022smart,bubeck2023sparks} \Ying{double-check}. Inspired by the powerful language modeling capabilities of LLMs, the question arises: \emph{``Can LLMs serve as Samantha-like personal companions in our daily life?''} \Ying{should clarify the terms: Samantha-like, personal companions.}

We argue that the answer today remains, ``Not without further capabilities''. Despite impressive human-like language capabilities, LLMs are hosted in a remote GPU cloud and unable to perceive the user's physical surroundings or daily experience. Without such personal context, it is difficult for LLMs to understand a user's personality, experiences, preferences, and habits \Ying{keep consistency. did we actually infer the four aspects? if yes, what are the details }. Today, LLMs behave more like knowledgable information sources with some reasoning capabilities, i.e., like a useful interface layer over Wikipedia. They don't yet behave like companions. We argue that lack of personal context is the main remaining challenge preventing LLMs from realizing the vision of Samantha \Ying{why?}. We categorize \emph{personal context} into three levels in the temporal dimension \Ying{why these three levels, and how they are proposed? e.g., from temporal dimensions? }.
\begin{itemize}

\item \textbf{Episodic context} includes on-going conversation, as well as the user's in-situ context such as current time, location, perceived visual scene, activity, as well as the user's emotional and mood conditions \Ying{what exactly they are?}. This information can help LLMs understand the underlying meanings of the user's speech \Ying{how about the information about the visual perception?} and generate relevant and appropriate responses. 
% \Ying{it is unclear for me what is ``relevant'' and  ``appropriate''? why the episodic context is key in generating relevant and appropriate responses?}  

\item \textbf{Historical context} is the historical summary of the past episodic context, which includes the user's past daily events and dialogue contents \Ying{exactly in the later method section?}. This information can help LLMs maintain the coherence and continuity of the dialogue, and avoid repeating or contradicting previous statements. 

\item \textbf{User profile} is distilled \Ying{how and why? what is the difference between it and the historical context} historical information related to the user's personality, preferences, social background, and life habits revealed during interaction with the dialogue system. It can enable LLMs to adapt to the user's personality and long-term goals with more consistent and anthropomorphic responses. 
% ***Double-check. I Changed ``preferences'' to ``goals'' here.***

\end{itemize}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.6\textwidth]{images/Our_system.pdf}
    \caption{Conceptual overview of OS-1 workflow. }
    \label{system_workflow}
\end{figure}

This work presents OS-1~\footnote{``OS-1'' was the name for Samantha's underlying implementation
in the movie ``Her".}, an intelligent eyewear with an LLM-based dialogue system to provide personalized conversations and daily companionship. 
As is shown in Figure~\ref{system_workflow}, the OS-1 eyewear perceives the user's in-situ visual and audio signals through the built-in camera and microphone, and the captured episodic contexts (sentences describing current user states) are analyzed and summarised by a vision-language model deployed in the cloud. 
Databases of historical contexts and personal profiles are constructed based on accumulated episodic contexts.
For each conversational cycle, OS-1 utilizes the latest episodic context as the key to retrieving the databases of historical context and user profile, and the retrieved information is synthesized and fed as LLM prompts to produce personalized responses.

To form personal context and generate personalized responses, OS-1 contains four main modules.
\begin{itemize}

    \item \textbf{Episodic context capture}. The smart eyewear captures the user's visual and voice surroundings and transfers them to the cloud on the fly. We extract the semantic description of images and transcribe voice data into text. Combining these two modalities, we infer the user's current activity,  location, as well as the user's emotional and mood conditions, which constitute the episodic context.
		
    \item \textbf{Historical context extraction}. To generate a historical summary of the episodic context, we design a clustering method to remove inter-episodic context redundancy and produce the historical context in the form of recapitulative event-level descriptions. Inspired by the memory organization structure of the human brain~\cite{de2021dimensions}, we design indexing methods along temporal, spatial, and semantic dimensions, which facilitate efficient retrieval of historical contexts from different perspectives.
		
    \item \textbf{User profile distillation}. We further infer the user's personality, preferences, social background, and life habits to form a user profile from the historical context. To address the bias or error of our inference of the user profile due to the limited interactions, we design an update scheme that checks and revises the previous user profile based on the current interaction with the users.
    % \Ying{Why can an update scheme help to address the issue of limited interaction?}
		
    \item \textbf{Personalized response generation}. Whenever a user starts a conversation, OS-1 retrieves the historical context from temporal, spatial, and semantic dimensions based on the current episodic context, and also retrieves the relevant user profile. The personal context containing these three contexts is used as an LLM prompt, providing personalized responses that are transmitted from the cloud to the smart eyewear's speakers.
		
\end{itemize}

% \textcolor{blue}{***It would be better to give the requirements for your system and the reasons for design decisioins before giving design details. What you did makes more sense in the context of why you did it.***}

% We conducted in-lab studies and in-field pilot studies to test the performance of OS-1 and its key components in terms of capturing, accumulating, and refining personal context, and to evaluate the implications of providing chatbots with personal context as a personal companion. 

We conducted in-lab studies and in-field pilot studies to test the performance of OS-1 with its core ability of capturing, accumulating, and refining personal context, and to evaluate the implications of providing chatbots with personal context as a personal companion.

In the in-lab study, we measure the performance of OS-1 with the ability to capture personal context, including episodic context extraction, historical context generation, and context retrieval. The results indicate that, compared with LLM-only methods, OS-1 delivers a significant improvement in generating personal context-aware responses with improvements in relevance score (28.57\%), personalization score (46.43\%), and engagement score (37.50\%).
% thod, with performance gains of 28.57\%, 46.43\%, and 37.50\%, respectively. 
This confirms our above statement that \emph{``LLMs cannot serve as personal companions in our daily life without further capabilities.''}

% relevance, personalization, and engagement

% ***If you can give a concrete, aggregate number, that is better than claiming improvement.*** 
% Furthermore, we used ChatGPT to simulate users with various personality traits who interact with OS-1. Evaluations with both simulated and real human participants demonstrate that incorporating personal context enhances personalization by ***\%.

% In the in-lab study, we designed three tasks to measure the performance of OS-1's key components, namely episodic context extraction, historical context generation, and context retrieval. The results indicate that our method
% ***I think you should replace ``our method'' with a short list of the key capabilites.*** 
% enable an accuracy improvement of***. 
% %***If you can give a concrete, aggregate number, that is better than claiming improvement.*** 
% Furthermore, we used ChatGPT to simulate users with various personality traits who interact with OS-1. Evaluations with both simulated and real human participants demonstrate that incorporating personal context enhances personalization by ***\%. 
% ***Can you report an aggregate number here based on your scales? That's more solid than a general claim of improvement.***


We conducted a 7-day pilot study with 10 participants to evaluate the effectiveness of OS-1 in engaging in personalized dialogue based on various scenarios. 
We assessed the degree of personalization of OS-1 using human evaluation on three metrics: relevance, personalization, and engagement. We also analyzed the system-generated utterances to examine how OS-1 can adapt to users' personalities, preferences, and habits over time. Our results show that by leveraging personal context OS-1 can effectively improve user satisfaction, engagement, and perceived personalization, and demonstrate its potential applicability in two inspiring personal service downstream applications -- emotional support and personal assistance.

Our work makes the following contributions.
\begin{enumerate}

\item We design and implement an always-available smart eyewear-LLM based personal dialogue system that captures the user's multi-modal surroundings on-the-fly, generates personal context, and engages in personalized conversation with the user.  \Ying{Additional: formulate the problem of ``personal context''  -- is it an important problem that has never been investigated previously? if yes, this part should be included in your contributions, instead of just describing a proposed method.}

\item We propose a novel method to capture, accumulate, and refine personal context from the user's multi-modal surroundings and dialogue history, and a multi-dimensional indexing and retrieval mechanism that integrates multiple personal contexts to generate personalized responses. Our method facilitates dynamic adaptation to the user's surroundings, experiences, and traits, enabling an engaging and customized conversation experience. 

\item We conducted an in-lab study and a pilot study to evaluate the impact of using personal context within the dialogue system. Our results show that it improves user satisfaction and engagement. We also demonstrate that OS-1 can distill accurate user profiles through personal, context-aware dialogue interactions, which can be used to support various personalized services and applications. 

\end{enumerate}

% ying: tech challenges?
